Survey on Memory-Augmented Neural Networks: Cognitive Insights to AI Applications

This paper explores Memory-Augmented Neural Networks (MANNs), delving into how they blend human-like memory processes into AI. It covers different memory types, like sensory, short-term, and long-term memory, linking psychological theories with AI applications. The study investigates advanced architectures such as Hopfield Networks, Neural Turing Machines, Correlation Matrix Memories, Memformer, and Neural Attention Memory, explaining how they work and where they excel. It dives into real-world uses of MANNs across Natural Language Processing, Computer Vision, Multimodal Learning, and Retrieval Models, showing how memory boosters enhance accuracy, efficiency, and reliability in AI tasks. Overall, this survey provides a comprehensive view of MANNs, offering insights for future research in memory-based AI systems.

==> 6-colab-strategy.tex <==
\section{Statement of Individual Contribution}
\textbf{Savya Khosla} is responsible for writing the section on memory-inspired neural architectures.

\textbf{Zhen Zhu} is responsible for writing the section on memory theories: from psychology to artificial intelligence.
% drafted Sec.~\ref{sec:memory_theories}.

\textbf{Yifei He} is responsible for writing the section on applications of memory-augmented neural networks and discussion about potential future research directions.
